Can Language Models be Biomedical Knowledge Bases?

Pre-trained language models (LMs) have become ubiquitous in solving various natural language processing (NLP) tasks. There has been increasing interest in what knowledge these LMs contain and how we can extract that knowledge, treating LMs as knowledge bases (KBs). While there has been much work on probing LMs in the general domain, there has been little attention to whether these powerful LMs can be used as domain-specific KBs. To this end, we create the BioLAMA benchmark, which is comprised of 49K biomedical factual knowledge triples for probing biomedical LMs. We find that biomedical LMs with recently proposed probing methods can achieve up to 18.51% Acc@5 on retrieving biomedical knowledge. Although this seems promising given the task difficulty, our detailed analyses reveal that most predictions are highly correlated with prompt templates without any subjects, hence producing similar results on each relation and hindering their capabilities to be used as domain-specific KBs. We hope that BioLAMA can serve as a challenging benchmark for biomedical factual probing.

==> tables/arc/decoding_ablation.tex <==
\begin{table}[]
    \centering
    \resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{lllll}
\toprule
\textbf{decoding} & \textbf{BERT} & \textbf{BioBERT} & \textbf{BioBERT-WWM} & \textbf{Bio-LM} \\
\midrule
independence & \textbf{2.41} & 3.51 & 3.33 & 11.76 \\
order & \textbf{2.41} & 3.57 & 3.98 & 11.90 \\
confidence & 1.65 & \textbf{3.82} & \textbf{5.02} & \textbf{12.13} \\
\bottomrule
\end{tabular}
    }\vspace{-0.1cm}
    \caption{Ablation study for three decoding strategies. Acc@1 in wikidata testset is reported. confidence-based decoding outperforms the other methods}\vspace{-0.0cm}\label{tab:ablation_decoding}
\end{table}

==> tables/arc/diversity.tex <==
\begin{table*}[]
    \centering
    \resizebox{1.95\columnwidth}{!}{%
\begin{tabular}{lll}
\toprule
 \textbf{pid(Acc@1, Acc@5)} & \textbf{subject} & \textbf{top5 predictions} \\
 \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}GP1\\ (16.80/37.66)\end{tabular}} & NRF1 & \textbf{metabolism}, signaling, signaling pathways, immune response, signal transduction \\
 & SLC19A3 & \textbf{metabolism}, signaling, signaling pathways, signal transduction, energy metabolism \\
 & OR52E6 & metabolism, signaling pathways, energy metabolism, development, \textbf{signal transduction} \\
 & GABBR2 & metabolism, signaling pathways, immune response, energy metabolism, \textbf{signal transduction} \\
 & TAS2R1 & metabolism, signaling pathways, immune response, \textbf{signal transduction}, energy metabolism \\
 \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}CP2\\ (17.88/18.02)\end{tabular}} & Furosemide & \textbf{cell death}, proliferation, programmed cell death, death, apoptosis \\
 & mocetinostat & \textbf{cell death}, proliferation, programmed cell death, apoptosis, death \\
 & Reactive Oxygen Species & \textbf{cell death}, programmed cell death, death, proliferation, apoptosis \\
 & 3-buten-2-one & \textbf{cell death}, proliferation, apoptosis, programmed cell death, cell proliferation \\
 & austenitic steel & cell death, proliferation, apoptosis, \textbf{cell proliferation}, programmed cell death \\
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}P2176\\ (5.57/21.90)\end{tabular}} & dysentery & \textbf{ciprofloxacin}, ethanol, cyclophosphamide, metronidazole, ciprofloxa \\
 & rheumatoid arthritis & \textbf{methotrexate}, cyclophosphamide, cyclophospha acetate, ciprofloxate, ciprofloxane \\
 & pure red-cell aplasia & \textbf{cyclophosphamide}, ethanol, methylprednisolone, rituximab, methotrexate \\
 & Kawasaki disease & cyclophosphamide, \textbf{aspirin}, immunoglobulin, ethanol, rituximab \\
 & amebiasis & ciprofloxacin, ciprofloxa, \textbf{metronidazole}, levofloxacin, zinc \\
 \bottomrule
\end{tabular}
    }\vspace{-0.1cm}
    \caption{Prediction diversity. \mujeen{need to quantify the diversity }}\vspace{-0.0cm}\label{tab:prediction_diversity}
\end{table*}




==> tables/arc/length_norm.tex <==
\begin{table}[]
    \centering
    \resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{lll}
\toprule
 \textbf{c} & \textbf{acc@1} & \textbf{prediction examples} \\
 \midrule
0 & \textbf{5.68} & AD, malaria, cisplatin, statins, ... \\
0.3 & 5.12 & jaundice,cyanosis, cyclosporine, ... \\
0.6 & 4.15 & insomnia, ... \\
1 & 3.49 & rheumatoid arthritis, hypotension, ... \\
\midrule
\textbf{Oracle length} & \textbf{16.75} & \\
\bottomrule
\end{tabular}
    }\vspace{-0.1cm}
    \caption{Ablation study for length normalization coefficient. 0 means no normalization and 1 means linear normalization.}\vspace{-0.0cm}\label{tab:ablation_length_norm}
\end{table}

==> tables/arc/manual_prompt_ablation.tex <==
\begin{table}[]
    \centering
    \resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{llcc}
\toprule
\textbf{pid} & \textbf{manual prompts} & \textbf{acc@1} & \textbf{acc@1 (ol)} \\
 \midrule
 \multirow{4}{*}{P2175} & [X] has effects on diseases such as [Y] & 2.61 & \textbf{9.15} \\
 & [X] cures diseases such as [Y] & \textbf{3.27} & 8.50 \\
 & [X] treats diseases such as [Y] & \textbf{3.27} & 7.84 \\
 & [X] reduces diseases such as [Y] & 2.61 & 5.23 \\
 \midrule
\multirow{3}{*}{P780} & [X] causes symptoms such as [Y] & \textbf{20.55} & \textbf{20.55} \\
 & [Y] is the most common symptom in [X] & 13.70 & \textbf{20.55} \\
 & [X] leads to symptoms such as [Y] & 15.07 & 16.44 \\
\bottomrule
\end{tabular}
    }\vspace{-0.1cm}
    \caption{Ablation study for manual prompts. `Acc@1 (ol)' refers to acc@1 with oracle entity length. We use BioBERT and `Acc@1 (ol)' to search for the best manual prompts based on the development set.}\vspace{-0.0cm}\label{tab:ablation_manual_prompt}
\end{table}




==> tables/arc/obj_type.tex <==
\begin{table}[]
    \centering
    \resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{lllll}
\toprule
\textbf{object} & \textbf{Acc@1} & \textbf{Acc@5} & \textbf{obj length} & \textbf{obj set size} \\
\midrule
\textbf{Chemical} & 24.60 & 43.27 & 4.91 & 1192 \\
\textbf{Symptoms} & 23.90 & 40.39 & 3.74 & 447 \\
\textbf{Pathway} & 16.80 & 17.25 & 6.61 & 1005 \\
\textbf{Phenotype} & 5.25 & 14.00 & 6.39 & 761 \\
\textbf{Disease} & 5.20 & 16.38 & 5.83 & 3171 \\
\textbf{Protein} & 0.02 & 3.73 & 3.65 & 3256 \\
\bottomrule
\end{tabular}
    }\vspace{-0.1cm}
    \caption{The performance of each object type. `obj length' refers to the number of tokens of unique object in test set and `obj set size' refers to the number of unique object. }\vspace{-0.0cm}\label{tab:obj_type}
\end{table}

==> tables/arc/plms.tex <==
\begin{table*}[]
    \centering
    \resizebox{1.95\columnwidth}{!}{%
\begin{tabular}{lllll}
\toprule
 & \textbf{Base LM} & \textbf{Corpus} &  \textbf{Vocab} & \textbf{Text Size} \\
 \midrule
\textbf{BERT}~\citep{devlin2019bert} & BERT & W+B  & W+B  & 3.3 words\\
\textbf{BioBERT}~\citep{lee2020biobert} & BERT & W+B+PubMed(Jan2019) & W+B & 4.5 words\\
% \textbf{BioBERT-WWM} & BERT & W+B+PubMed(Jan2019) & Word & W+B \\
\textbf{Bio-LM}~\citep{lewis2020pretrained} & RoBERTa & W+B+PubMed(Mar2020) & PubMed\\
\bottomrule
\end{tabular}
    }\vspace{-0.1cm}
    \caption{Comparision of PLMs \jinhyuk{base LM - BERT? RoBERTA? Corpus size? (BioBERT uses both Wiki + Pubmed)}\jinhyuk{large? base? maybe we need to add one large model to our exp} \mujeen{pretraining corpus date also matters}}\vspace{-0.0cm}\label{tab:compare_plms}
\end{table*}

==> tables/arc/prompts.tex <==
\begin{table*}[]
    \centering
    \resizebox{1.95\columnwidth}{!}{%
\begin{tabular}{ll}
\toprule
\textbf{Method} & \textbf{Prompt example} \\
\midrule
Manual~\citep{petroni2019language} & [Methotrexate] has effects on diseases such as [Y] \\
Manual (+synonym) & [Methotrexate], [Amethopterin], [Mexate], has effects on diseases such as [Y] \\
\midrule
Mined~\citep{jiang2020can} & [Methotrexate] in the treatment of chronic [Y]\\
\midrule
Optiprompt~\citep{zhong2021factual} & [Methotrexate] [V]$_1$ [V]$_2$ [V]$_3$ [V]$_4$ [V]$_5$ [Y] \\
Optiprompt (manual) & [Methotrexate] [V]$_1$:=has [V]$_2$:=effects \dots [V]$_6$ :=as [Y] \\
\bottomrule
\end{tabular}
    }\vspace{-0.1cm}
    \caption{Comparison of five prompts on relation P2175. Note that `Amethopterin' and `Mexate' are the synonym of the subject `Methotrexate'.
    \mujeen{need to make this look better or merge this to another table}\jinhyuk{add example and citation, maybe refer to how optiprompt show this} }\vspace{-0.0cm}\label{tab:compare_prompts}
\end{table*}

==> tables/arc/result_for_types.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.90\columnwidth}{!}{%
    \begin{tabular}{lcccccc}
        \toprule

        \textbf{Object types} & \textbf{Majority} & \textbf{IE} & \textbf{Bio-LM} \\
        
        \midrule
        
        chemical (935) & 2.93 & \textbf{20.75} & \ul{ 9.68} \\
        
        symptom (1157) & \ul{ 8.79} & 0.33 & \textbf{9.31} \\
        
        vertebrate (678) & \ul{ 6.05} & 0.59 & \textbf{6.93} \\
        
        disease (9555) & \ul{ 6.39} & \textbf{8.34} & 5.21 \\
        
        protein (3836) & \textbf{10.12} & \ul{ 7.66} & 3.68 \\
        
        pathway (887) & \textbf{15.90} & \ul{ 4.51} & 3.27 \\
        
        \bottomrule
    \end{tabular}
    }% vspace{-0.2cm}
    \caption{Acc@1 of each object type. The numbers in paraentheses refer to the number of samples for each object type.
    \mujeen{need to update}}
    \vspace{-0.2cm}\label{tab:result_for_type}
\end{table}

==> tables/arc/table.tex <==
% need clean up

\begin{table}[t]
    \centering
    \resizebox{0.95\columnwidth}{!}{%
    \begin{tabular}{lcccccc}
        \toprule
 &  \multicolumn{2}{c}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Dev}} & \multicolumn{2}{c}{\textbf{Test}} \\
\textbf{PID} & \textbf{Single} & \textbf{Multi} & \textbf{Single} & \textbf{Multi} & \textbf{Single} & \textbf{Multi} \\
\midrule
\textbf{P2175}  & 127 & 539 & 33 & 133 & 145 & 688 \\
\textbf{P2176} & 38 & 420 & 6 & 109 & 47 & 526 \\
\textbf{P2293} & 123 & 1145 & 25 & 292 & 141 & 1445 \\
\textbf{P3354} & 0 & 110 & 0 & 27 & 1 & 137 \\
\textbf{P3355} & 0 & 70 & 0 & 17 & 0 & 88 \\
\textbf{P769} & 15 & 24 & 3 & 7 & 19 & 30 \\
\textbf{P780} & 151 & 158 & 29 & 48 & 180 & 207 \\
        \bottomrule
    \end{tabular}
    }\vspace{-0.1cm}
    \caption{Single and multi token split data stats }\vspace{-0.0cm}\label{tab:single_multi_data_stats}
\end{table}



\begin{table}[t]
    \centering
    \resizebox{0.95\columnwidth}{!}{%
    \begin{tabular}{lccc}
        \toprule
\textbf{PID} & \textbf{All} & \textbf{Single} & \textbf{Multi} \\
\midrule
\textbf{P2175} & 7.20 & - & - \\
\textbf{P2176} & 11.34 & - & - \\
\textbf{P2293} & 3.03 & - & - \\
\textbf{P3354} & 0.00 & - & - \\
\textbf{P3355} & 0.00 & - & - \\
\textbf{P769} & 10.20 & - & - \\
\textbf{P780} & 33.08 & - & - \\
\midrule
\textbf{avg} & 9.26 & - & - \\
        \bottomrule
    \end{tabular}
    }\vspace{-0.1cm}
    \caption{Experiments using single, multi token datasets respectively. Acc@1 }\vspace{-0.0cm}\label{tab:experiment_single_multi}
\end{table}

\begin{table}[t]
    \centering
    \resizebox{0.95\columnwidth}{!}{%
    \begin{tabular}{lcc}
        \toprule
\textbf{PID} & \textbf{$\sim$2018} & \textbf{2019$\sim$2021} \\
\midrule
\textbf{P2175} & 1324 & 1 \\
\textbf{P2176} & 879 & 2 \\
\textbf{P2293} & 1852 & 18 \\
\textbf{P3354} & 99 & 1 \\
\textbf{P3355} & 59 & 1 \\
\textbf{P769} & 83 & 0 \\
\textbf{P780} & 598 & 2 \\
\midrule
\textbf{all} & 4894 & 25 \\
        \bottomrule
    \end{tabular}
    }\vspace{-0.1cm}
    \caption{Time-based split dataset}\vspace{-0.0cm}\label{tab:time_based_split}
\end{table}

